XGSwap: eXtreme Gradient boosting Swap for Routing in NISQ Devices

In the current landscape of noisy intermediate-scale quantum (NISQ) computing, the inherent noise presents significant challenges to achieving high-fidelity long-range entanglement. Furthermore, this challenge is amplified by the limited connectivity of current superconducting devices, necessitating state permutations to establish long-distance entanglement. Traditionally, graph methods are used to satisfy the coupling constraints of a given architecture by routing states along the shortest undirected path between qubits. In this work, we introduce a gradient boosting machine learning model to predict the fidelity of alternative--potentially longer--routing paths to improve fidelity. This model was trained on 4050 random CNOT gates ranging in length from 2 to 100+ qubits. The experiments were all executed on ibm_quebec, a 127-qubit IBM Quantum System One. Through more than 200+ tests run on actual hardware, our model successfully identified higher fidelity paths in approximately 23% of cases.

==> Tables/overall_degradation.tex <==
% \begin{figure*}[ht]
% \centering


% % \begin{subfigure}[t]{\textwidth}
% % \centering
% % \caption{}
% % \vspace{0.1in}
% %     \scalebox{0.65}{

% % \begin{tabular}{|c|cc|cc|cc|}
% % \hline
% % \rowcolor[HTML]{C0C0C0} 
% % \cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} }                                        & \multicolumn{2}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \textbf{2021}}}                                                       & \multicolumn{2}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \textbf{2022}}}                                                       & \multicolumn{2}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \textbf{2023}}}                                                       \\ \cline{2-7} 
% % \rowcolor[HTML]{C0C0C0} 
% % \multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \textbf{Backend Name}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \textbf{Readout Error}}} & {\color[HTML]{000000} \textbf{CNOT Error}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \textbf{Readout Error}}} & {\color[HTML]{000000} \textbf{CNOT Error}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \textbf{Readout Error}}} & {\color[HTML]{000000} \textbf{CNOT Error}} \\ \hline
% % ibm\_algiers                                                                           & \multicolumn{1}{c|}{0.03 $\pm$ 0.052}                                                         & 0.045 $\pm$ 0.16                              & \multicolumn{1}{c|}{0.035 $\pm$ 0.073 ( 18.4\% )}                                             & 0.063 $\pm$ 0.201 ( 39.7\% )                  & \multicolumn{1}{c|}{0.028 $\pm$ 0.045 ( -20.9\% )}                                            & 0.116 $\pm$ 0.24 ( 84.8\% )                   \\ \hline
% % ibm\_cairo                                                                             & \multicolumn{1}{c|}{0.021 $\pm$ 0.016}                                                        & 0.056 $\pm$ 0.023                             & \multicolumn{1}{c|}{0.017 $\pm$ 0.018 ( -18.9\% )}                                            & 0.099 $\pm$ 0.243 ( 78.6\% )                  & \multicolumn{1}{c|}{0.019 $\pm$ 0.019 ( 11.1\% )}                                             & 0.105 $\pm$ 0.259 ( 5.6\% )                   \\ \hline
% % ibmq\_kolkata                                                                          & \multicolumn{1}{c|}{0.012 $\pm$ 0.009}                                                        & 0.018 $\pm$ 0.027                             & \multicolumn{1}{c|}{0.019 $\pm$ 0.022 ( 53.4\% )}                                             & 0.057 $\pm$ 0.156 ( 214.6\% )                 & \multicolumn{1}{c|}{0.024 $\pm$ 0.027 ( 24.8\% )}                                             & 0.167 $\pm$ 0.332 ( 191.5\% )                 \\ \hline
% % \end{tabular}
% % }
% % \end{subfigure}
% \begin{subfigure}[t]{\textwidth}
%         \setlength\fboxsep{0pt}
%     \setlength\fboxrule{0.0pt}

% \fbox{\includegraphics[width=7in]{Figures/cnot_error_graph.pdf}}
% \end{subfigure}
% \caption{Smoothed Average CNOT Error Over Time with Standard Deviation, illustrating the temporal evolution of CNOT errors for select backends. Data collected using Qiskit  \cite{treinish_qiskitqiskit-metapackage_2023} in January 2024.}

% \end{figure*}
